Active Third-Person Imitation Learning

We consider the problem of third-person imitation learning with the additional challenge that the learner must select the perspective from which they observe the expert. In our setting, each perspective provides only limited information about the expert's behavior, and the learning agent must carefully select and combine information from different perspectives to achieve competitive performance. This setting is inspired by real-world imitation learning applications, e.g., in robotics, a robot might observe a human demonstrator via camera and receive information from different perspectives depending on the camera's position. We formalize the aforementioned active third-person imitation learning problem, theoretically analyze its characteristics, and propose a generative adversarial network-based active learning approach. Empirically, we demstrate that our proposed approach can effectively learn from expert demonstrations and explore the importance of different architectural choices for the learner's performance.

==> a15_hopper_results.tex <==
\timo{This is commented out. We can add it back in for the rebuttal}
\section{Results for the Hopper Environment}\label{app:results_hopper}
The following part of this paper describes our findings for the MuJoCo Hopper environment \cite{brockman2016openai}. For a description of how we define the perspectives, please refer to Appendix~\ref{app:hopper:details}. Figure~\ref{fig:hopper:results} shows the results on Hopper when examining different perspective selection strategies and levels of available information. We find that except for the \textsc{UCB} strategy, none of the proposed strategies can improve their performance in terms of environment reward throughout the training (cf.\ Figure~\ref{fig:hopper:results:strategies}). Regarding different levels of available information, the results depicted in Figure~\ref{fig:hopper:results:information} indicate that the \textsc{Best} active perspective selection strategy offers similar performance to having \textsc{Full} information, albeit at the cost of having a higher variance. 

One hypothesis for Hopper's lack of learning progress might be the environment's complexity. Compared to Point and Reacher, the action space of Hopper has an additional dimension. Hopper also has the most complex reward function out of all our evaluated environments, making it difficult to implicitly learn about the reward function via expert imitation. Additionally, we hypothesize that our particular set of hyperparameters, in conjunction with the used seeds, was particularly well-suited for the \textsc{UCB} strategy. Due to computational constraints, we searched for hyperparameters only for the active perspective selection scenario. Further hyperparameter tuning might  improve the results for the other strategies and the \textsc{Full}/\textsc{Partial} information settings.

In Figure~\ref{fig:hopper:correlation_strategies}, we visualize whether attempting to learn correlations between perspectives can be harmful for Hopper. With one notable exception (\textsc{UCB}), the findings validate our results from the main paper that correlation learning is generally not harmful.

\begin{figure}
  \subcaptionbox{Hopper strategies\label{fig:hopper:results:strategies}}[.5\linewidth]{%
    \includegraphics[width=70mm,scale=0.5]{figures/neurips_experiments/hopper_bands_strategy.pdf}%
  }%
  \hfill
  \subcaptionbox{Hopper information\label{fig:hopper:results:information}}[.5\linewidth]{%
    \includegraphics[width=70mm,scale=0.5]{figures/neurips_experiments/hopper_bands_information.pdf}%
  }
    \caption{Results for the Hopper environment. \emph{(\subref{fig:hopper:results:strategies})} shows the learning curves for our perspective selection strategies. None can significantly improve throughout the training except for the \textsc{UCB} strategy. \emph{(\subref{fig:hopper:results:information})} visualizes results for different levels of available information. The \textsc{Best} perspective selection strategy can approximate the performance of having \textsc{Full} information. \textsc{Partial} information yields the worst results.
    }
  \label{fig:hopper:results}
\end{figure}

\begin{figure}
  \centering
    \subcaptionbox*{Hopper correlation learning}[1\linewidth]{%
    \includegraphics[width=70mm,scale=0.5]{figures/neurips_experiments/hopper_bands_strategy_corr_plain.pdf}%
  }
    \caption{Effect of correlation learning for Hopper. Except for the \textsc{UCB} strategy, correlation learning without highly correlated/duplicate perspectives does not harm the agent's performance.}
  \label{fig:hopper:correlation_strategies}
  
\end{figure}

\clearpage

==> a16_additional_figures.tex <==
\section{Additional Figures}\label{app:additional_figures}
This section presents additional figures corroborating the results of the main paper's experiments (Section~\ref{sec:experiments}). Unless stated otherwise, all plots use the same settings as the ones stated in the experiments section of the main paper. Figure~\ref{fig:correlated_perspectives_point} implies that learning correlations is not harmful even when perspectives are independent. We evaluate this claim in the default specifications of the Point and Reacher environments as defined in Appendix~\ref{app:point:details} and~\ref{app:reacher:details}. Figure~\ref{fig:corr_plain_shaded_bands} shows the training curves for the \textsc{MinProb}, \textsc{MaxProb}, \textsc{UCB} and \textsc{Random} strategies. Indeed, we find the very similar performance of strategies irrespective of correlation learning regarding final reward.

\begin{figure}
  \subcaptionbox{Point}[.5\linewidth]{%
    \includegraphics[width=70mm,scale=0.5]{figures/neurips_experiments/point_bands_strategy_corr_plain.pdf}%
  }%
  \hfill
  \subcaptionbox{Reacher}[.5\linewidth]{%
    \includegraphics[width=70mm,scale=0.5]{figures/neurips_experiments/reacher_bands_strategy_corr_plain.pdf}%
  }
    \caption{Effect of correlation learning in the default environment configurations for Point and Reacher. We find no consistent and significant effect on an agent's final performance.}
  \label{fig:corr_plain_shaded_bands}
\end{figure}

One possible conjecture for the superior performance of correlation learning in the Duplicate Point environment may be fewer selections of the no-information perspective. We examine this hypothesis in Figure~\ref{fig:duplicate_point_perspective_bars}. The bar plots show the relative frequency with which perspectives are selected for data generation. Contrary to our working hypothesis, we do not find a substantial difference in selection frequencies for the no-information perspective. However, the plots show that learning correlations produce a better balance between partially informative perspectives. We conjecture that learning about correlations may lead to the agent being able to combine information among perspectives with partial information in a more efficient manner.

\begin{figure}
\label{fig:correlated_perspectives_point:learning_curves_appendix}
\includegraphics[width=70mm,scale=0.5]{figures/neurips_experiments/point_bands_strategy_corr.pdf}%
  \hfill
\caption{The plot shows the same learning curves for correlation/no correlation learning as the main paper in Figure~\ref{fig:correlated_perspectives_point:learning_curves}.}

\end{figure}

\begin{figure}
  \subcaptionbox{No correlation learning\label{fig:correlated_perspectives_point:bar_no_corr}}[.5\linewidth]{%
    \includegraphics[width=70mm,scale=0.5]{figures/neurips_experiments/point_duplicate_bar_corr_False.pdf}%
  }%
  \hfill
  \subcaptionbox{Correlation learning\label{fig:correlated_perspectives_point:bar_corr}}[.5\linewidth]{%
    \includegraphics[width=70mm,scale=0.5]{figures/neurips_experiments/point_duplicate_bar_corr_True.pdf}%
  }
    \caption{Selected perspectives for expert data generation on the Duplicate Point environment using all seeds. Learning correlations does not result in a substantially decreased frequency for the no-information perspective except for the \textsc{MaxProb} strategy. However, correlation learning leads to a more balanced selection of perspectives with partial information.}
  \label{fig:duplicate_point_perspective_bars}

\end{figure}



\clearpage

==> a17_perspective_selection_studies.tex <==
\timo{This should be adapted to show that the best strategy is more effective at selecting non-useless perspectives}
\timo{Remove the references to hopper here}
\section{Effect of Perspective Selection Strategies}

In our penultimate section, we provide additional information about how the perspective selection strategies affect the chosen discriminator over the course of the training.
Our working hypothesis before conducting the experiments was the following: As there is no distinction possible between the expert's and the learner's policy using the non-informative perspective, the discriminator will assign a probability of $50\%$ irrespective of whether the data was generated by the expert or the learner. Note that in our algorithm the learner policy is trained after optimizing the discriminators. In our eyes, this should lead to the discriminators assigning a lower reward to both partial information perspectives as they have learned to distinguish between the expert's and learner's data distribution. 

Having discussed our hypothesis on how the perspective selection strategy affects discriminator selection, we expect to find that \textsc{MinProb} and \textsc{UCB} (except for some exploration) should always choose the perspective where the discrepancy between the learner's policy and the expert is largest. A hypothetical consequence of our analysis is that \textsc{MinProb} and \textsc{UCB} should be the best strategies. On the other hand, \textsc{MaxProb} should mostly choose the non-informative perspective as it returns the highest reward signal once discriminators are sufficiently well optimized.

\timo{Remove Hopper references here}
\begin{table}[htp] %
\caption{Percentage of chosen strategy for each discriminator: \textit{Partial information 1} refers to Figures~\ref{fig:point:x}, \ref{fig:reacher:x}, \ref{fig:hopper:x}; \textit{Partial information 2} refers to \ref{fig:point:y}, \ref{fig:reacher:y}, \ref{fig:hopper:y}.\\}
\label{tab:strategy}
\centering
\begin{tabular}{clccc} 
    \toprule
    \textbf{Env} & \textbf{Perspective} & \textsc{MaxProb} & \textsc{MinProb} & \textsc{UCB} \\
    \midrule
    & Partial Info 1  & $4.48\% \pm 9.46 \%$ & $45.38\% \pm 50.70 \%$ & \hspace{1.5pt} $39.77\% \pm 28.29 \%$ \\
    \textbf{Point} & Partial Info 2 & $15.38\% \pm 12.90 \%$ & $24.69\% \pm 43.87 \%$ & \hspace{1.5pt} $36.79\% \pm 27.18 \%$ \\
    & No Info & $80.13\% \pm 15.70 \%$ & $29.94\% \pm 46.92 \%$ & \hspace{1.5pt} $23.44\% \pm 18.08 \%$ \\[2mm]
    & Partial Info 1  & $30.57\% \pm 35.51 \%$ & $32.71\% \pm 41.67 \%$  & $31.45\% \pm 9.28 \%$ \\
    \textbf{Reacher} & Partial Info 2 & $18.39\% \pm 17.05 \%$  & $29.68\% \pm 43.20 \%$  &  $39.89\% \pm 8.26 \%$ \\
    & No Info & $51.04\% \pm 31.63 \%$ & $37.60\% \pm 45.98 \% $ & $28.72\% \pm 7.16 \%$ \\[2mm]
    & Partial Info 1  & $22.50\% \pm 40.54\%$ & $18.42\% \pm 35.28\%$ & $16.70\% \pm 7.31\% $ \\
    \textbf{Hopper} & Partial Info 2 &  $11.28\% \pm 22.60\% $ & $19.30\% \pm 35.28\% $ & \hspace{2.5pt} $46.65\% \pm 15.07\%$ \\
    & No Info &  $66.22\% \pm 40.96 \% $ & $62.28\% \pm 43.39\%$ & \hspace{2.5pt} $36.66 \% \pm 12.21\%$ \\
    \bottomrule
    
\end{tabular}
\end{table}

In Table~\ref{tab:strategy}, we summarize the relative per-episode frequencies for each perspective the agent uses to generate its rewards. We indicate one standard deviation for all frequencies and omit the \textsc{Random} strategy as it uses uniform discriminator selection by definition. The results in Table~\ref{tab:strategy} confirm our hypothesis that the \textsc{MaxProb} strategy is particularly susceptible to selecting the no-information perspective, with the effect being strongest for Point. We observe that \textsc{MinProb} and \textsc{MaxProb} exhibit high variance for their frequencies. We attribute this to the fact that both strategies tend to lock into specific perspectives throughout the training, cf.\ Figure~\ref{fig:reward_perspectives_min_max}. The degree and speed with which this lock-in occurs depend on the particular environment, strategy, and initially collected data (i.e., seed). 


We cannot find such a noticeable association for the other environments, leading us to the following informal conjecture: Periodically selecting the no-information perspective synchronizes the learner's and discriminators' current training status. This implicitly balances the discriminator's capabilities with the learner's current imitation progress, allowing for learning.

\begin{figure}
  \subcaptionbox{\textsc{MaxProb}\label{fig:reward_perspectives:matrix_maxprob}}[.5\linewidth]{%
    \includegraphics[width=70mm,scale=0.5]{figures/neurips_experiments/reacher_heatmap_MaxProb_worst.pdf}%
  }%
  \hfill
  \subcaptionbox{\textsc{MinProb}\label{fig:reward_perspectives:matrix_minprob}}[.5\linewidth]{%
    \includegraphics[width=70mm,scale=0.5]{figures/neurips_experiments/reacher_heatmap_MinProb_best.pdf}%
  }
    \caption{\emph{(\subref{fig:reward_perspectives:matrix_maxprob})} Selected perspectives for the best performing run of the \textsc{MaxProb} strategy. After initially selecting the front perspective until iteration 19, the agent converges to only choosing the no-information discriminator to generate its reward. \emph{(\subref{fig:reward_perspectives:matrix_minprob})} For the best-performing run using the \textsc{MinProb} strategy, the agent rarely chooses the no-information perspective for reward generation as it provides no discriminatory signal.
    }
  \label{fig:reward_perspectives_min_max}
\end{figure}

\begin{figure}
  \centering
    \subcaptionbox*{\textsc{UCB}}[1\linewidth]{%
    \includegraphics[width=70mm,scale=0.5]{figures/neurips_experiments/reacher_heatmap_BEST_ucb.pdf}%
  }
    \caption{Visualization of the best-performing run on reacher using the \textsc{UCB} strategy. After an initial exploration phase, \textsc{UCB} converges to using the side perspective. Frequencies for the no-information perspective drop after 25 iterations.}
  \label{fig:reward_perspectives_ucb}
  
\end{figure}

We use the best runs for a particular strategy on Reacher to visualize the selected perspectives for the agent's reward generation in Figures~\ref{fig:reward_perspectives_min_max} and~\ref{fig:reward_perspectives_ucb}. For the \textsc{MaxProb} strategy in Figure~\ref{fig:reward_perspectives:matrix_maxprob}, we can see how the agent initially selects the front perspective before converging to only choosing the no-information perspective. This is consistent with the hypothesis outlined in the previous paragraphs, namely that the no-information discriminator will end up being the one indicating the highest probability of being an expert as training of the other discriminators progresses. In contrast, the \textsc{MinProb} (Figure~\ref{fig:reward_perspectives:matrix_minprob}) and \text{UCB} (Figure~\ref{fig:reward_perspectives_ucb}) strategies rarely select the uninformative perspective. \textsc{MinProb} mostly selects the front perspective whereas \text{UCB} explores initially before converging to the side perspective.



==> a19_notes.tex <==
\section*{Setting}

\begin{itemize}
    \item Known $A_L$. Easy, just pick greedily to minimize teaching risk. Complication $w^*$ not known.
\end{itemize}


\section*{Extensions for NeurIPS}

\textbf{Theory}
\begin{itemize}
  \item \todo{Optimal strategies for stylized setting.} Known covariance matrix of feature expectations; Which knowledge regarding reward function? (probably none); Regret minimization; Extension of teaching risk setting? (because each view now also provides information about other views)

  \item \todo{Optimal strategies for less stylized settings.} Estimation of covariance matrix needs to be performed. => Sample complexity.

  \item \todo{??? Setting: Where we have a "new" final perspective during execution.}

  \item \todo{Negative results: are single perspectives good enough? }
\end{itemize}


\textbf{Experiments}
\begin{itemize}
  \item Proof of concept experiments in toy setting.

  \item \todo{Transition to challenging 3rd person setting.} Can we relate discriminators to correlation? Probably not in the current form. Discriminators are independent.

  \item \todo{Proper 3rd person setting}
\end{itemize}


\section{Results}

\subsection{Learning About Feature-correlations}

\begin{itemize}



  \item \textbf{Setting of a non-linear reward function. Conjunction  features.}
    Same issues as for non-linear feature transformations arise.

    $\Rightarrow$ How to deal with this:
    \begin{itemize}
        \item[\checked] Theoretical: Example of an unbounded relative increase in error because of not matching the joint features
        \item Is there a good characterization of performance loss?
        \item Practical: Enable switching the perspective during execution? Align demonstrations recorded from different perspectives? Illustrate the importance of having good perspectives. 
        \item Possible structure in the case of non-linear reward functions regarding the features $R(\phi) = Linear(Nonlinear(perspective1), nonlinear(perspective2), ...)$
        \item Relate to teaching risk?
    \end{itemize}

      
\end{itemize}

\subsection{Feature matching in individual perspectives does not ensure good performance}

 


    \begin{theorem}
        Even in cases in which feature matching is sufficient to guarantee optimal performance, imperfect feature matching can result in large errors, i.e., there exists an MDP and perspectives such that $\| A_\nu\Psi - A_\nu\Psi^E \| \leq \epsilon$ but $\frac{R(\Psi^E) - R(\Psi)}{R(\Psi^E)} \rightarrow 1$.
    \end{theorem}
    \begin{proof}
        An example in which feature important for reward is downscaled versus other features are not. 
    \end{proof}

    + connect with teaching risk.


\subsection{Characterization of performance loss}

\begin{itemize}
    \item Performance loss increases with down-scaling of features relevant for reward.
    \item Performance loss increases with non-linearities in the reward.
    \item Optimal performance achievable if all correlations are presented in the perspectives.
\end{itemize}



\subsection{Algorithmic exploitation of structure}
\begin{itemize}
    \item For bandits we consider the eigenvalues of 
      $$V_t = \lambda I + \sum_{t=1}^T A_{\nu_t}^T A_{\nu_t}$$
      to select the next best perspective.
    \item What is the impact of $A_\nu$ on the correlation structure of feature observations (which we can estimate)?
      \begin{align*}
          (A_1 \phi)^T (A_2 \phi') = \phi^T A_1^T A_2 \phi'.
      \end{align*}
      Taking the expectation:
      \begin{align*}
          \Psi^E A_1^T A_2 \Psi^E
      \end{align*}
      Hence there is some relevant information in the feature correlations, mixed with the feature expectations.
      How does the multiplication with $\Psi$ transform the correlations?

      $\Rightarrow$ Empirical evaluation ("pseudo" MDP, real tabular MDP).
\end{itemize}


\subsection{Experiments}

\begin{itemize}
    \item Illustrate query strategies in "pseudo MDPs" + grid worlds.
    \item Illustrate performance limits in tailored MDP variants.
    \item Illustrate scalability to real-world using discriminator framework.

\end{itemize}

\subsection{TODO}

\begin{itemize}
    \item Add layer to discriminators to allow exploiting correlations.
    \item Consequences of aspects limiting performance?

    \item Revise introduction + problem setting $\Rightarrow$ critical review by Adish
\end{itemize}



\subsection{Future}

\begin{itemize}
    \item Also being able to pick different experts. ($\rightarrow$ contextualization?)
\end{itemize}




\subsection{A Bandit Perspective}

Formalization as bandit.

\begin{itemize}
    \item Action space = (set of policies, characterized by their state-action-distribution) $\times$ (perspective) -> set of policies is a polyhedron

    \item Observation = difference of feature expectations of chosen policy to expert's policy in the respective dimension (or 0-1 feedback depending on match/no-match)

    \todo{+ consider the case where we only see the mismatch for a single demonstration}

    \item Goal: Minimize 
\end{itemize}

\todo{Alternative formulation?} Only choose perspective. How does the policy come about?

\todo{? Base policy from GAIL. + $\epsilon$-greedy}

$$\Psi(\pi) = F \mu(\pi)$$

$$\| F_\nu \mu(\pi) - F_\nu \mu(\pi^*) \|$$

\todo{Simulate noise of single making single observations.}

\begin{itemize}
    \item Finish mapping to linear bandits
    \item Implement toy examples
    \item Transfer theory inspired strategy to a practical setting
\end{itemize}

\subsection{Optimal Strategies Knowing the Learner's Perspectives (+$A^L$)}




\subsection{Setting 1}

\begin{itemize}
    \item Arms correspond to the different perspectives, $A\nu$ is known
    \item Observations are of single demonstrations, i.e., mean feature expectations + noise, i.e., $A_\nu\Psi^E + \epsilon$   %
    \item The expert's feature expectations are unknown.
    \item The goal is to infer the $\Psi^E$ as well as possible. 
\end{itemize}

$\Rightarrow$ select perspectives to minimize distance to true parameters (using bounds from linear bandits)

In practice not realizable, as $A_\nu$ is not known.
In general, we can't learn about $A_nu$ by only making observations from it.
Maybe it is better to also play a policy to make inference.

\includegraphics[width=10cm]{figures/queries.pdf}

$$x = A_\nu \Psi(\pi) - A_\nu \Psi^E$$

\begin{itemize}
  \item Without inferring $A_\nu$.

  \item Available: $a_\nu = A_\nu \Psi(\pi)$ for any perspective $\nu$ and any policy of our choice $\pi$.

  \item $\Rightarrow$ Compute correlation structure (at a particular time $t$ for policy $\pi_t$) and leverage it for selecting perspectives.

  \item Algorithmically: 
    Exploit "cluster structure" in perspectives + current errors to improve + diversity (more globally).

  \item $a_\nu = (A_\nu F) \mu(\pi)$

    $a_\nu^E = A_\nu F \mu(\pi^E)$

  \item Baselines:
     UCB (not exploiting correlation structure), uniform (not considering errors and structure)

  \item Use $A_\nu$ to scale errors
  
\end{itemize}


$$A_\text{First person} \Psi(\pi)$$

\subsection{@Timo}

\begin{itemize}
    \item Reproduce results in our considered setting
\end{itemize}

\input{algorithms/algorithm-old.tex}

\section{TODO}

\begin{itemize}
    \item \todo{Replace "Novice" with "Learner".}
    \item \todo{Have a contextual view? At least in future work.}
    \item \todo{Applications?}
    \item \todo{Deep net structure}
    \item \todo{Experiments}
    \item \todo{Generalize Theorem~\ref{thm:linear-rewards-and-projections} to account for different feature matching precisions in the different dimensions.}
    \item Figure 1: \todo{Use cameras to illustrate the idea better? Or even put some plots from later here?}
    \item Intro: \todo{Think deeper about contextulaization.}
\end{itemize}

\begin{itemize}
    \item 1.5 pages: Introduction
    \item 1.0 pages: Problem Setting
    \item 1.5 pages: Analysis and Insights; theory; 
current 4.1 is a standalone section
    \item 1.8 pages: Our Approach
Warm up/motivation
approach (include current section 4.2)
    \item 2.3 pages: Experimental Evaluation
      \begin{itemize}
        \item Figure 1: Environments / Perspectives in one row
        \item Figure 2: (one plot per environment)
Comparison of strategies including baselines (single perspective, super-perspective, etc.)
        \item Figure 3:  (one plot per environment)
Ablations:
Our best technique vs. no-shared layer vs. shared-layer without perspective information)
(optional) 
        \item Figure 4:
Illustration of the selected perspectives
      \end{itemize}
    \item 0.7 pages: Related work
    \item 0.2 pages: Conclusions
\end{itemize}


==> algorithms/algorithm-old.tex <==

\begin{algorithm2e}[H]
\caption{Active Third-person  Imitation Learning}\label{alg:one}
\SetAlgoLined
\DontPrintSemicolon
\KwIn{perspective selection strategy $\strategy$, number of iterations $K$, perspectives $\perspectives$, horizon $\horizon$, time shift $\Delta$, trajectories for discriminator training $E_d$, training epochs for  policy $E_p$, batch size discriminator $b_d$, batch size policy $b_p$}
\tcc{Initialisation}
\For{$\perspective \in \perspectives$}{
    Initialise discriminator $\discriminator_\perspective$
}
Initialise environment $\environment$\;
Initialise expert policy $\pi^\expert$ and learner policy $\pi^\learner_\theta$  \;
Initialise perspective selection strategy $\strategy$\;
Initialise policy improvement algorithm $\trainalgo$\;
\tcc{training: each iteration first trains the discriminators, then the learner policy}
\For{$i=1,\ldots,K$}{
   \tcc{Get demonstrations from expert}
   Collect samples $\omega^\expert$ from $\pi^\expert$ from $E_d$ epochs \;
    \tcc{Get demonstrations from learner}
    Collect samples $\omega^\learner$ from  $\pi^\learner$ from $E_d$ epochs\;
    \tcc{Update discriminators}
    \For{$\discriminator \in \{ \discriminator_\perspective | \perspective \in \perspectives \}$}{
        Prepare batches $\Tilde{\omega}^\expert$, $\Tilde{\omega}^\learner$ of observation tuples $o_t,o_{t+\Delta}$ with batch size $b_d$\;
        \ForEach{ $\Tilde{\omega}^\expert$, $\Tilde{\omega}^\learner$}{ 
          $\mathcal{L}=\CE(\discriminator(\Tilde{\omega}^\expert),\textnormal{"expert"})$ \;
          minimize $\mathcal{L}$ with ADAM \;
          $\mathcal{L}=\CE(\discriminator(\Tilde{\omega}^\learner),\textnormal{"learner"}))$ \;
          minimize $\mathcal{L}$ with ADAM \; %
        }
    }
    \tcc{Train learner policy}
    \For{$e=1,\ldots,E_p$}{
    Collect samples $\omega^\learner$ from $\pi^\learner$ of batch size $b_p$\;
    Prepare $\Tilde{\omega}^\learner$ by storing tuples $o_t,o_{t+\Delta}$ \;
    Select discriminator $\discriminator$ according to $\strategy$ \;
    rewards = $-\log(\discriminator$($\Tilde{\omega}^\learner))$\;
    Train the learner policy $\pi^\learner$  with the rewards from the discriminator via $\trainalgo$ \;
    }%
}%
\KwResult{Optimized learner policy $\pi^\learner$} %
\end{algorithm2e}


